Phase-Field Modeling of Fracture for Ferromagnetic Materials through Maxwell's Equation

Electro-active materials are classified as electrostrictive and piezoelectric materials. They deform under the action of an external electric field. Piezoelectric material, as a special class of active materials, can produce an internal electric field when subjected to mechanical stress or strain. In return, there is the converse piezoelectric response, which expresses the induction of the mechanical deformation in the material when it is subjected to the application of the electric field. This work presents a variational-based computational modeling approach for failure prediction of ferromagnetic materials. In order to solve this problem, a coupling between magnetostriction and mechanics is modeled, then the fracture mechanism in ferromagnetic materials is investigated. Furthermore, the failure mechanics of ferromagnetic materials under the magnetostrictive effects is studied based on a variational phase-field model of fracture. Phase-field fracture is numerically challenging since the energy functional may admit several local minima, imposing the global irreversibility of the fracture field and dependency of regularization parameters related discretization size. Here, the failure behavior of a magnetoelastic solid body is formulated based on the Helmholtz free energy function, in which the strain tensor, the magnetic induction vector, and the crack phase-field are introduced as state variables. This coupled formulation leads to a continuity equation for the magnetic vector potential through well-known Maxwell's equations. Hence, the energetic crack driving force is governed by the coupled magneto-mechanical effects under the magneto-static state. Several numerical results substantiate our developments.

==> Figures/fig-potatoes/fig.tex <==
\begin{figure}[!htb]
%\unitlength1.0cm
\begin{center}
  %
  \psfrag{B}      [r][r]{$\calB$}
  \psfrag{lc}     [c][c]{$l_d$} 
  \psfrag{x}      [l][l]{$\Bx\in\calB$}  
  \psfrag{bb}     [l][l]{$\bar\Bb$}
  \psfrag{nd}     [l][l]{$\Bn$}
  \psfrag{n}      [r][r]{$\Bn$}
  \psfrag{t}      [r][r]{$\bar{\Bt}=\bar{\Bsigma} \cdot \Bn$}
  \psfrag{Gamma}  [c][c]{$\Gamma$}
  \psfrag{ubar}   [r][r]{$\Bu=\bar{\Bu}$}
  \psfrag{Abar}   [r][r]{$\BA=\bar{\BA}$}
  \psfrag{ndn0}   [c][c]{$\nabla{d} \cdot \Bn=0$}
  \psfrag{A0}     [l][l]{$\bar{\BA}=\textbf{0}$}
  \psfrag{Omega}  [c][c]{$\Omega$}
  \psfrag{u}      [c][c]{$\Bu$}
  \psfrag{d}      [c][c]{$d$}
  \psfrag{A}      [c][c]{$\BA$}
  \psfrag{p}      [c][c]{$+$}
  \psfrag{ng}     [c][c]{$-$}
  \psfrag{N}      [l][l]{$\BN$}
  \psfrag{dOmega} [l][l]{$\partial{\Omega}$}
  \psfrag{vacuum} [c][c]{Vacuum}
  %%
%
%%\includegraphics[width=11.875cm,height=4cm]{\DIR/fig.eps}
\includegraphics[width=\textwidth]{\DIR/fig.eps}
\end{center}
%\abovecaptionskip-1mm
\caption{Primary variable fields in magneto-elasticity, for a solid
  body $\calB \subset \calR^{d}$ with dimension $d \in [2,3]$. $(a)$
  The displacement field $\Bu$ defined on $\calB$ and Neumann-type
  boundary condition for traction $\bar{\Bt}=\bar{\Bsigma} \cdot
  \Bn$. $(b)$ The magnetic vector potential $\BA$ in $\Omega$ that is
  continuous across the interface $\partial{\calB}$,
  i.e. $\llbracket \BA \rrbracket:\BA^{+}-\BA^{-}=0$ on
  $\partial{\calB}$, and zero on the boundary $\partial{\Omega}$ free
  space box (vacuum). $(c)$ The crack phase-field is determined by
  Dirichlet-type boundary condition $d=1$ on $\Gamma$ and Neumann-type
  boundary condition $\nabla d \cdot \Bn = 0$ on the full surface $\partial{\calB}$.}
\label{\LABEL}
\end{figure}


==> M.tex <==
In the formulation of coupling magneto-mechanical model with the
phase-field approach, the permeability of the solid body is computed
as a function of the crack phase-field, it means that when cracks
propagate in the body, the cracking paths get contact with the free
space. Therefore, the magnetic field decreases along the cracking
paths, which consequently causes the magnetization to get
decreased. Thus, we have the following relations for the magnetic
field and the magnetization along the crack geometries
\begin{equatio}
  \BB \to \textbf{0} \quad \AND \quad \BB \to \textbf{0}
\end{equation}


==> makefile <==
#-----------------------------------------------------------------------------
#   Makefile for LaTeX
#------------------------------------------------------------------------------
# set compiler options

# set the names of the compilers
TEX = latex
BIB = bibtex
DVI = dvips
PDF = ps2pdf
#
SOURCE = main
# compile changed objects
ref:
	bibtool -s -d ref_0.bib -o ref.bib && bibtex main

all: ref dvi ps pdf

# dvi: 
# 	$(TEX) $(SOURCE) 
# 	$(TEX) $(SOURCE) 
# 	$(TEX) $(SOURCE) 

dvi: 
	$(TEX) $(SOURCE) 
	$(BIB) $(SOURCE) 
	$(TEX) $(SOURCE) 
	$(TEX) $(SOURCE) 

ps: 
	$(DVI) -Ppdf -t a4paper -o $(SOURCE).ps $(SOURCE)

see:
	okular $(SOURCE).pdf &
#	gv  $(SOURCE).pdf &
#	gv  $(SOURCE).ps &

pdf: 
	$(PDF) $(SOURCE).ps 

#
clean: 
	rm -f $(SOURCE).dvi \
	rm -f $(SOURCE).aux \
	rm -f $(SOURCE).out \
	rm -f $(SOURCE).toc \
	rm -f $(SOURCE).bbl \
	rm -f $(SOURCE).blg \
	rm -f $(SOURCE).log \
	rm -f $(SOURCE).ps \
	rm -f $(SOURCE).pdf \
	rm -f *~ ref.bib
file:
	$(TEX) $(SOURCE) && make ps && make pdf	

latex:
	make clean && make all && clear
	@@echo "---> LATEX: IT IS READY!!"


==> note.tex <==
\TODO{Nima, CORRECTION SEC. 2.2}
 For the variational formulation setting, it suffices to define the constitutive energy density functions $W_{elas}$, $W_{plas}$, and $W_{fluid}$ to establish the multi-field evolution problem in terms of the primary fields. As we shall recall in the sequel, such a variational structure is not always present in phase-field models for ductile fracture, resulting in greater flexibility at the cost of  a convenient mathematical structure.
 
 In this section, we presents a theoretical development associated with the failure mechanism of the ferromagnetic  material regarding their fully coupled magneto-mechanical  characteristics based on the variational phase-field model. To this  end, the governing equations and the related constitutive relations corresponding the boundary value problem are proposed on the basis of the energy-based magneto-mechanical model. To do so, a coupling between  the magnetostriction and the mechanics is formulated to investigate the mechanical deformation of the material under the magnetic forces then the cracking response under the magnetic forces is examined. We complete this section, by providing the theoretical framework for magnetostrcitively-induced cracking as a compact algorithmic framework.
 
 
 Next, we use (29) as a departure point for the Global-Local approach in Section 3. 
 

 As we shall recall in the sequel
 
 
 %
 The constitutive equation is additively split to purely tensile contribution  ${\bm \sigma}^{+}({\bm{\varepsilon}})$ and purely compression contribution ${\bm \sigma}^{-}({\bm{\varepsilon}})$, reads
 %
 \begin{equation}
 	{\bm \sigma}(\bm{\varepsilon},s ):=\frac{\partial w_{bulk}(\Bve, s)}{\partial {\bm \varepsilon}} = g(s_+)\frac{\partial \widetilde{\Psi}^{+}}{\partial \bm \varepsilon}+\frac{\partial \widetilde{\Psi}^{-}}{\partial \bm \varepsilon}
 	=g(s_+){\bm {\widetilde{\sigma}}^{+}}+{\bm {\widetilde{\sigma}}^{-}},
 	\label{eq232_7}
 \end{equation}
